In-Context Unlearning: Language Models as Few Shot Unlearners

Machine unlearning, the study of efficiently removing the impact of specific training instances on a model, has garnered increased attention in recent years due to regulatory guidelines such as the \emph{Right to be Forgotten}. Achieving precise unlearning typically involves fully retraining the model and is computationally infeasible in case of very large models such as Large Language Models (LLMs). To this end, recent work has proposed several algorithms which approximate the removal of training data without retraining the model. These algorithms crucially rely on access to the model parameters in order to update them, an assumption that may not hold in practice due to computational constraints or having only query access to the LLMs. In this work, we propose a new class of unlearning methods for LLMs called ``In-Context Unlearning.'' This method unlearns instances from the model by simply providing specific kinds of inputs in context, without the need to update model parameters. To unlearn specific training instances, we present these instances to the LLMs at inference time along with labels that differ from their ground truth. Our experimental results demonstrate that in-context unlearning performs on par with, or in some cases outperforms other state-of-the-art methods that require access to model parameters, effectively removing the influence of specific instances on the model while preserving test accuracy.

==> tex/tables/table_accuracy.tex <==
% OLD VERSION: 3 commas
% \begin{table}[htb!]
% \centering
% \resizebox{0.49\textwidth}{!}{%
% \begin{tabular}{cccccccc}
% \toprule
% \multirow{2}{*}{Dataset} &  \multirow{2}{*}{Method} & \multicolumn{3}{c}{Bloom 560M} & \multicolumn{3}{c}{Bloom 1.1B}   \\
% \cmidrule(l){3-5} \cmidrule(l){6-8} 
% & & Train & Forget & Test & Train & Forget & Test \\
% \cmidrule(lr){1-1} \cmidrule(r){2-2} \cmidrule(l){3-5} \cmidrule(l){6-8} 
% \multirow{3}{*}{Amazon} & \cellcolor{gray!22} \texttt{ICUL(4)} & \cellcolor{gray!22} $0.933 \pm 0.012$ & \cellcolor{gray!22} $\textbf{0.930} \pm 0.012$ & \cellcolor{gray!22} $0.918 \pm 0.013$ & \cellcolor{gray!22} $0.955 \pm 0.007$ & \cellcolor{gray!22} $\textbf{0.953} \pm 0.010$ & \cellcolor{gray!22} $0.939 \pm 0.005$ \\
% & \cellcolor{gray!22} \texttt{GA(1e-05)} & \cellcolor{gray!22} $\textbf{0.959} \pm 0.002$ & \cellcolor{gray!22} $0.918 \pm 0.012$ & \cellcolor{gray!22} $\textbf{0.940} \pm 0.002$ & \cellcolor{gray!22} $\textbf{0.966} \pm 0.001$ & \cellcolor{gray!22} $0.920 \pm 0.003$ & \cellcolor{gray!22} $\textbf{0.948} \pm 0.001$ \\
% & \texttt{Baseline} & $0.960 \pm 0.002$ & $0.960 \pm 0.002$ & $0.940 \pm 0.002$ & $0.967 \pm 0.001$ & $0.967 \pm 0.001$ & $0.949 \pm 0.002$ \\
% \cmidrule(l){1-8} 
% \multirow{3}{*}{Yelp} & \cellcolor{gray!22} \texttt{ICUL(4)} & \cellcolor{gray!22} $0.942 \pm 0.027$ & \cellcolor{gray!22} $\textbf{0.940} \pm 0.028$ & \cellcolor{gray!22} $0.936 \pm 0.015$ & \cellcolor{gray!22} $0.964 \pm 0.009$ & \cellcolor{gray!22} $\textbf{0.962} \pm 0.012$ & \cellcolor{gray!22} $0.958 \pm 0.006$ \\ 
% & \cellcolor{gray!22} \texttt{GA(1e-05)} & \cellcolor{gray!22} $\textbf{0.974} \pm 0.001$ & \cellcolor{gray!22} $\textbf{0.944} \pm 0.010$ & \cellcolor{gray!22} $\textbf{0.958} \pm 0.003$ & \cellcolor{gray!22} $\textbf{0.979} \pm 0.001$ & \cellcolor{gray!22} $0.947 \pm 0.003$ & \cellcolor{gray!22} $\textbf{0.966} \pm 0.002$ \\
% & \texttt{Baseline} & $0.974 \pm 0.001$ & $0.974 \pm 0.001$ & $0.958 \pm 0.003$ & $0.980 \pm 0.001$ & $0.980 \pm 0.001$ & $0.966 \pm 0.002$ \\
% \cmidrule(l){1-8} 
% \multirow{3}{*}{SST-2} & \cellcolor{gray!22} \texttt{ICUL(6)} & \cellcolor{gray!22} $0.870 \pm 0.035$ & \cellcolor{gray!22} $\textbf{0.856} \pm 0.035$ & \cellcolor{gray!22} $0.835 \pm 0.030$ & \cellcolor{gray!22} $0.925 \pm 0.018$ & \cellcolor{gray!22} $\textbf{0.903} \pm 0.016$ & \cellcolor{gray!22} $0.881 \pm 0.015$ \\
% & \cellcolor{gray!22} \texttt{GA(1e-05)} & \cellcolor{gray!22} $\textbf{0.951} \pm 0.004$ & \cellcolor{gray!22} $0.845 \pm 0.020$ & \cellcolor{gray!22} $\textbf{0.909} \pm 0.003$ & \cellcolor{gray!22} $\textbf{0.965} \pm 0.002$ & \cellcolor{gray!22} $0.860 \pm 0.007$ & \cellcolor{gray!22} $\textbf{0.919} \pm 0.002$ \\
% &  \texttt{Baseline} & $0.953 \pm 0.004$ &  $0.953 \pm 0.004$ &  $0.911 \pm 0.002$ &  $0.966 \pm 0.002$ & $0.966 \pm 0.002$ & $0.920 \pm 0.002$ \\
% \bottomrule
% \end{tabular}
% }
% \caption{\textbf{Classification accuracy (CA).} CA on train, forget and test points across all data sets and model sizes.
% While \texttt{GA} always has more favorable test accuracy, the performance gap between \texttt{ICUL} and \texttt{GA} on test data becomes smaller as we increase model size despite \texttt{ICUL} having no access to model parameters.}
% \label{tab:ubs1_performance_accuracy}
% \vspace{-0.5cm}
% \end{table}

\begin{table}[tb]
\centering
\resizebox{0.49\textwidth}{!}{%
\begin{tabular}{cccccccc}
\toprule
\multirow{2}{*}{Dataset} &  \multirow{2}{*}{Method} & \multicolumn{3}{c}{Bloom 560M} & \multicolumn{3}{c}{Bloom 1.1B}   \\
\cmidrule(l){3-5} \cmidrule(l){6-8} 
& & Train & Forget & Test & Train & Forget & Test \\
\cmidrule(lr){1-1} \cmidrule(r){2-2} \cmidrule(l){3-5} \cmidrule(l){6-8} 
\multirow{3}{*}{A} & \cellcolor{gray!22} \texttt{ICUL(4)} & \cellcolor{gray!22} $0.933 \pm 0.01$ & \cellcolor{gray!22} $\textbf{0.930} \pm 0.01$ & \cellcolor{gray!22} $0.918 \pm 0.01$ & \cellcolor{gray!22} $0.955 \pm 0.01$ & \cellcolor{gray!22} $\textbf{0.953} \pm 0.01$ & \cellcolor{gray!22} $0.939 \pm 0.01$ \\
& \cellcolor{gray!22} \texttt{GA(1e-05)} & \cellcolor{gray!22} $\textbf{0.959} \pm 0.00$ & \cellcolor{gray!22} $0.918 \pm 0.01$ & \cellcolor{gray!22} $\textbf{0.940} \pm 0.00$ & \cellcolor{gray!22} $\textbf{0.966} \pm 0.00$ & \cellcolor{gray!22} $0.920 \pm 0.00$ & \cellcolor{gray!22} $\textbf{0.948} \pm 0.00$ \\
& \texttt{Baseline} & $0.960 \pm 0.00$ & $0.960 \pm 0.00$ & $0.940 \pm 0.00$ & $0.967 \pm 0.00$ & $0.967 \pm 0.00$ & $0.949 \pm 0.00$ \\
\cmidrule(l){1-8} 
\multirow{3}{*}{Y} & \cellcolor{gray!22} \texttt{ICUL(4)} & \cellcolor{gray!22} $0.942 \pm 0.03$ & \cellcolor{gray!22} $\textbf{0.940} \pm 0.03$ & \cellcolor{gray!22} $0.936 \pm 0.02$ & \cellcolor{gray!22} $0.964 \pm 0.01$ & \cellcolor{gray!22} $\textbf{0.962} \pm 0.01$ & \cellcolor{gray!22} $0.958 \pm 0.01$ \\ 
& \cellcolor{gray!22} \texttt{GA(1e-05)} & \cellcolor{gray!22} $\textbf{0.974} \pm 0.00$ & \cellcolor{gray!22} $\textbf{0.944} \pm 0.01$ & \cellcolor{gray!22} $\textbf{0.958} \pm 0.00$ & \cellcolor{gray!22} $\textbf{0.979} \pm 0.00$ & \cellcolor{gray!22} $0.947 \pm 0.00$ & \cellcolor{gray!22} $\textbf{0.966} \pm 0.00$ \\
& \texttt{Baseline} & $0.974 \pm 0.00$ & $0.974 \pm 0.00$ & $0.958 \pm 0.00$ & $0.980 \pm 0.00$ & $0.980 \pm 0.00$ & $0.966 \pm 0.00$ \\
\cmidrule(l){1-8} 
\multirow{3}{*}{S} & \cellcolor{gray!22} \texttt{ICUL(6)} & \cellcolor{gray!22} $0.870 \pm 0.04$ & \cellcolor{gray!22} $\textbf{0.856} \pm 0.04$ & \cellcolor{gray!22} $0.835 \pm 0.03$ & \cellcolor{gray!22} $0.925 \pm 0.02$ & \cellcolor{gray!22} $\textbf{0.903} \pm 0.02$ & \cellcolor{gray!22} $0.881 \pm 0.02$ \\
& \cellcolor{gray!22} \texttt{GA(1e-05)} & \cellcolor{gray!22} $\textbf{0.951} \pm 0.00$ & \cellcolor{gray!22} $0.845 \pm 0.02$ & \cellcolor{gray!22} $\textbf{0.909} \pm 0.00$ & \cellcolor{gray!22} $\textbf{0.965} \pm 0.00$ & \cellcolor{gray!22} $0.860 \pm 0.01$ & \cellcolor{gray!22} $\textbf{0.919} \pm 0.00$ \\
&  \texttt{Baseline} & $0.953 \pm 0.00$ &  $0.953 \pm 0.00$ &  $0.911 \pm 0.00$ &  $0.966 \pm 0.00$ & $0.966 \pm 0.00$ & $0.920 \pm 0.00$ \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Classification accuracy (CA)} on train, forget and test points across all data sets and model sizes.
While \texttt{GA} always has more favorable test accuracy, the performance gap between \texttt{ICUL} and \texttt{GA} on test data narrows down as we increase model size which is remarkable as \texttt{ICUL} has no access to model parameters.}
\label{tab:ubs1_performance_accuracy}
\vspace{-0.5cm}
\end{table}

==> tex/tables/table_tprs.tex <==
\begin{figure*}[htb]
\centering
% \begin{subfigure}{\textwidth}
% \centering
% \includegraphics[width=\textwidth]{figures/info_extraction_loglog_bloom-560m_icl_ubs1_vary_lfmfirst-k_lr1e-05_minkeep2.pdf}
% \caption{Bloom (560M parameters)}
% \label{fig:ubs1_roc_bloom560}
% \end{subfigure}
% \vfill
\begin{subfigure}{\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/info_extraction_loglog_bloom-1b1_icl_ubs1_vary_lfmfirst-k_lr1e-05_minkeep2.pdf}
%\caption{Bloom (1.1B parameters)}
%\label{fig:ubs1_roc_bloom1b1}
\end{subfigure}
\caption{\textbf{Unlearning sucess} across different unlearning methods for different datasets for an underlying Bloom 1.1B LLM using log scaled ROC curves.
The closer to the diagonal the better, which amounts to the adversary randomly guessing whether a given point is (still) part of the model or not.
For the green and red curves, \texttt{LiRA-Forget} is run against the updated models $\bar{f}$, which were updated using \texttt{GA} (solid red) or \texttt{ICUL} (dashdot green).
The black dashed line represents the \texttt{baseline} of not removing the point where the same attack is run on the model $\ftheta$, as described in Section \ref{sec:eval_measures}.
The numbers in brackets denote the best parameters and the numbers after that show the AUC $\pm 1$ standard deviation across 10 runs.  
Shades indicate $\pm 1$ standard deviation across 10 runs.}
\label{fig:ubs1_unlearning_success}
\end{figure*}

% \begin{table*}[htb!]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{clcggcgg}
% \toprule
% \multirow{2}{*}{Dataset} & \multirow{2}{*}{Metric} & \multicolumn{3}{c}{Bloom 560M} &  \multicolumn{3}{c}{Bloom 1.1B} \\
% \cmidrule(l){3-5} \cmidrule(l){6-8}
% & & \texttt{Baseline} & \texttt{ICUL} & \texttt{GA} & \texttt{Baseline} & \texttt{ICUL} & \texttt{GA}  \\
% \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(l){3-5} \cmidrule(l){6-8}
% \multirow{4}{*}{Amazon} & AUC & $0.5420 \pm 0.0040$ & $\textbf{0.5060} \pm 0.0049$ & $0.5870 \pm 0.0149$ & $0.5570 \pm 0.0090$ & $\textbf{0.5220} \pm 0.0108$ & $0.6740 \pm 0.0410$ \\
% & $\text{TPR}_{.001}$ & $0.0043 \pm 0.0016$ & $0.0013 \pm 0.0006$ & $\textbf{0.0008} \pm 0.0004$ & $0.0046 \pm 0.0011$ & $\textbf{0.0015} \pm 0.0008$ & $0.0017 \pm 0.0007$ \\
% & $\text{TPR}_{.01}$ & $0.0251 \pm 0.0028$ & $0.0114 \pm 0.0030$ & $\textbf{0.0106} \pm 0.0017$ & $0.0300 \pm 0.0019$ & $\textbf{0.0112} \pm 0.0037$ & $0.0173 \pm 0.0038$ \\
% & $\text{TPR}_{.1}$ & $0.1403 \pm 0.0046$ & $\textbf{0.1028} \pm 0.0141$ & $0.1491 \pm 0.0082$ & $0.1536 \pm 0.0124$ & $\textbf{0.0986} \pm 0.0161$ & $0.2164 \pm 0.0446$ \\
% \cmidrule(lr){1-8}
% \multirow{4}{*}{Yelp} & AUC & $0.5690 \pm 0.0430$ & $\textbf{0.5030} \pm 0.0110$ & $0.6590 \pm 0.0584$ & $0.5580 \pm 0.0183$ & $\textbf{0.5090} \pm 0.0181$ & $0.6790 \pm 0.0552$  \\
%  & $\text{TPR}_{.001}$ & $0.0068 \pm 0.0037$ & $\textbf{0.0010} \pm 0.0004$ & $0.0021 \pm 0.0012$ & $0.0074 \pm 0.0016$ & $\textbf{0.0006} \pm 0.0004$ & $0.0014 \pm 0.0006$ \\
% & $\text{TPR}_{.01}$ & $0.0323 \pm 0.0111$ & $\textbf{0.0100} \pm 0.0037$ & $0.0219 \pm 0.0095$ & $0.0339 \pm 0.0093$ & $\textbf{0.0085} \pm 0.0038$ & $0.0182 \pm 0.0054$ \\
% & $\text{TPR}_{.1}$ & $0.1768 \pm 0.0482$ & $\textbf{0.0968} \pm 0.0211$ & $0.2423 \pm 0.0820$ & $0.1622 \pm 0.0291$ & $\textbf{0.0893} \pm 0.0198$ & $0.2507 \pm 0.0750$ \\
% \cmidrule(lr){1-8}
% \multirow{4}{*}{SST-2} & AUC & $0.5610 \pm 0.0030$ & $\textbf{0.5050} \pm 0.0067$ & $0.5930 \pm 0.0100$ & $0.5840 \pm 0.0049$ & $\textbf{0.5300} \pm 0.0077$ & $0.5940 \pm 0.0049$  \\
% & $\text{TPR}_{.001}$ & $0.0030 \pm 0.0010$ & $0.0015 \pm 0.0002$ & $\textbf{0.0009} \pm 0.0004$ & $0.0039 \pm 0.0008$ & $\textbf{0.0016} \pm 0.0007$ & $\textbf{0.0016} \pm 0.0003$ \\
% & $\text{TPR}_{.01}$ & $0.0250 \pm 0.0021$ & $\textbf{0.0113} \pm 0.0016$ & $0.0118 \pm 0.0013$ & $0.0313 \pm 0.0027$ & $\textbf{0.0134} \pm 0.0020$ & $0.0137 \pm 0.0010$ \\
% & $\text{TPR}_{.1}$ & $0.1551 \pm 0.0043$ & $\textbf{0.1032} \pm 0.0065$ & $0.1441 \pm 0.0067$ & $0.1751 \pm 0.0080$ & $\textbf{0.1165} \pm 0.0119$ & $0.1436 \pm 0.0065$ \\
% \bottomrule
% \end{tabular}
% }
% \caption{\textbf{Unlearning success} at or below false positive rates of $10^{-1}$ across unlearning methods. 
% We report $\text{TPR}_{x}$, which measures the \text{TPR} at $\text{FPR} = x$, for different datasets and model sizes.
% Additionally, we report AUC, which denotes the area under the receiver operating characteristic curve.
% The results are averaged over 10 evaluation runs and include $\pm 1$ standard deviation.}
% \label{tab:overiew_table}
% %\vspace{-0.0cm}
% \end{table*}

